Can LLMs Master Math? Investigating Large Language Models on Math Stack Exchange

Large Language Models (LLMs) have demonstrated exceptional capabilities in various natural language tasks, often achieving performances that surpass those of humans. Despite these advancements, the domain of mathematics presents a distinctive challenge, primarily due to its specialized structure and the precision it demands. In this study, we adopted a two-step approach for investigating the proficiency of LLMs in answering mathematical questions. First, we employ the most effective LLMs, as identified by their performance on math question-answer benchmarks, to generate answers to 78 questions from the Math Stack Exchange (MSE). Second, a case analysis is conducted on the LLM that showed the highest performance, focusing on the quality and accuracy of its answers through manual evaluation. We found that GPT-4 performs best (nDCG of 0.48 and P@10 of 0.37) amongst existing LLMs fine-tuned for answering mathematics questions and outperforms the current best approach on ArqMATH3 Task1, considering P@10. Our Case analysis indicates that while the GPT-4 can generate relevant responses in certain instances, it does not consistently answer all questions accurately. This paper explores the current limitations of LLMs in navigating complex mathematical problem-solving. Through case analysis, we shed light on the gaps in LLM capabilities within mathematics, thereby setting the stage for future research and advancements in AI-driven mathematical reasoning. We make our code and findings publicly available for research: \url{https://github.com/gipplab/LLM-Investig-MathStackExchange}

==> prev_caseStudy.tex <==
\section{Case study}

For the case study, we selected questions we wanted to analyze with GPT-4.
The selection was done by observing questions for which GPT-4 boosts retrieval and the ones for which DPR has better retrieval performance than GPT-4.

\subsection{GPT-4}
% We observe that GPT-4 can produce correct answers for many topics from the dataset. 
% GPT-4 gave similar evaluation scores as the best-performing method, showcasing its ability to generate relevant content. 
% However, there remain a lot of wrong answers. 
% In the following, we present two topics, one for which GPT-4's answer retrieved accepted answers and one where the retrieved answer is not accepted. 
In the following, we present two topics, one for which querying GPT-4's answer boosts retrieval in terms of P@10 and one where retrieval is worsened. 
The cases we study should be considered outliers: For most topics in the dataset, we observe differences in P@10 scores from between $-0.1$ (GPT-4 answers outperformed by original DPR run) to $0.2$ (GPT-4 answers outperforming original DPR run).
We do not mention answers due to space limitations but all the recorded answers for GPT-4~\footnote{\url{https://anonymous.4open.science/r/LLMsForArqmath-6A0C/topics-and-qrels/topics.arqmath-2022-gpt4-generated-answers.csv}} and all the other LLMs are available in the repository.
%\subsubsection{A.310: Wrong answer}
%\fbox{%
%  \parbox{0.5\textwidth}{
%	Find the positive integer solutions for: $\frac{4}{x} + \frac{10}{y} = 1$ \\ I had calculated the solutions manually but it was a very tedious process. Is there any better way to do this?
% }%
%}

\subsubsection{\href{https://math.stackexchange.com/questions/4022815/what-does-this-bracket-notation-mean/1958336\#1958336}{A.384}: Retriveal Boost}
% GPT-4 correctly answers a question:\\
% \fbox{%
%   \parbox{0.47\textwidth}{I am currently taking MIT6.006 and I came across this problem on the problem set. Despite the fact I have learned Discrete Mathematics before, I have never seen such notation before, and I would like to know what it means and how it works, Thank you: $$ f_3(n) = \binom n2$$(Transcribed from screenshot)
%   }
% }
% This is not surprising since an answer does not involve mathematical reasoning.
\begin{figure}
    \centering
    \begin{tcolorbox}[standard jigsaw,opacityback=0,left=1pt, right=0pt, top=1pt, bottom=0pt, code={\singlespacing}]
    I am currently taking MIT6.006, and I came across this problem on the problem set. Despite the fact I have learned Discrete Mathematics before, I have never seen such notation before, and I would like to know what it means and how it works, Thank you: $$ f_3(n) = \binom n2$$
    \end{tcolorbox}
    \caption{Question which is correctly answered by GPT-4. We do not include the generated answer.}
    \label{fig:gptcorrect}
\end{figure}

The question shown in Figure~\ref{fig:gptcorrect}, GPT-4's answer strongly shows increases P@10 (from 0.0 of DPR to 0.6 of GPT-4).
The reason is that the first retrieved results by the DPR do not feature a binomial coefficient at all, but the first results of the GPT-4 retrieved result include at least an expansion of $\binom n2$. 
We observe that, without context, DPR cannot infer any meaning from the formula. 
Hence, GPT-4 shows a good contextual understanding of the ground truth formula.
% MABOWDOR corrects this problem using its structural search engine (Precision@10 is elevated to 0.4.).

\subsubsection{\href{https://math.stackexchange.com/questions/4155217/suppose-that-all-the-tangent-lines-of-a-regular-plane-curve-pass-through-some-fi?noredirect=1&lq=1}{A.337}: retrival Worsened}

\begin{figure}
    \centering
    \begin{tcolorbox}[standard jigsaw,opacityback=0,left=1pt, right=0pt, top=1pt, bottom=0pt, code={\singlespacing}]
    \textbf{Question.} Suppose that all the tangent lines of a regular plane curve pass through some fixed point. Prove that the curve is part of a straight line. Prove the same result if all the normal lines are parallel. I am working on differential geometry from the book by Pressley and I have a doubt in the solution of the above question whose (brief) solution is given by: \textbf{Solution:} We can assume that the curve $\gamma$ is unit-speed and that the tangent lines all pass through the origin (by applying a translation to $\gamma$). Then, there is a scalar$\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$. Then, $\gamma '' = \lambda'\gamma   + \lambda \gamma' = (\lambda' + \lambda^2)\gamma$. Can anyone please explain me how does this line follow : " Then, there is a scalar $\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$." Thanks in advance.
    \end{tcolorbox}

    \begin{tcolorbox}[standard jigsaw,opacityback=0,left=1pt, right=0pt, top=1pt, bottom=0pt, code={\singlespacing}]
    \textbf{Reason for worsened retrieval.} Imagine a car driving along the curve, and at the point of interest, the car hits an oil slick and shoots off in the straight line of its travel as it hits the point. The line of the car gives the tangent line at the point (provided the curve is differentiable at the point). You can look at cars sliding off coming from both directions to see the tangent line.
    \end{tcolorbox}



    % \begin{tcolorbox}[standard jigsaw,opacityback=0]
    % \textbf{Answer.} Certainly! To understand the line "Then, there is a scalar $\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$", we must delve into some differential geometry concepts.  Given a unit-speed curve $\gamma(t)$ in the plane, its tangent vector at any point is $\gamma'(t)$. The statement that all tangent lines pass through a fixed point (in this case, the origin after translation) means that every tangent vector is a scalar multiple of the position vector of the curve at that point.  Let's break it down:  1. **Tangent Vector**: The tangent vector to a curve at a point is a vector that "touches" the curve at that point and points in the direction in which the curve is going. For a unit-speed curve $\gamma(t)$, the tangent vector is given by $\gamma'(t)$.  2. **Position Vector**: The position vector of a point on the curve, relative to the origin, is simply $\gamma(t)$.  3. **Scalar Multiple**: Saying that the tangent vector is a scalar multiple of the position vector means there exists some scalar function $\lambda(t)$ such that $\gamma'(t) = \lambda(t) \gamma(t)$.  This relationship indicates that at every point on the curve, the direction in which the curve is moving (the tangent vector) is directly along the line from the origin to that point on the curve (the position vector), scaled by some factor $\lambda(t)$.  In simpler terms, if you draw a line from the origin to any point on the curve, the curve at that point is moving directly along this line, either towards or away from the origin, depending on the sign of $\lambda(t)$.   This behavior is characteristic of a straight line emanating from the origin. Hence, the curve must be part of a straight line.
    % \end{tcolorbox}
    
    \caption{Question which is incorrectly answered by GPT-4}
    \label{fig:extractedTOIs}
\end{figure}


P@10 decreases from 0.5 for the DPR run to 0.1 for GPT-4 for the following question (only title is shown, due to length):\\
% \fbox{%
%   \parbox{0.47\textwidth}{
% 		\textbf{Question.} Suppose that all the tangent lines of a regular plane curve pass through some fixed point. Prove that the curve is part of a straight line. Prove the same result if all the normal lines are parallel. I am working on differential geometry from the book by Pressley and I have a doubt in the solution of the above question whose (brief) solution is given by: \textbf{Solution:} We can assume that the curve $\gamma$ is unit-speed and that the tangent lines all pass through the origin (by applying a translation to $\gamma$). Then, there is a scalar$\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$. Then, $\gamma '' = \lambda'\gamma   + \lambda \gamma' = (\lambda' + \lambda^2)\gamma$. Can anyone please explain me how does this line follow : " Then, there is a scalar $\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$." Thanks in advance. 
%   }
% }
% \fbox{%
%   \parbox{0.47\textwidth}{
% Certainly! To understand the line "Then, there is a scalar $\lambda(t)$ such that $\gamma'(t) = \lambda(t)\gamma(t)$ for all $t$", we must delve into some differential geometry concepts.  Given a unit-speed curve $\gamma(t)$ in the plane, its tangent vector at any point is $\gamma'(t)$. The statement that all tangent lines pass through a fixed point (in this case, the origin after translation) means that every tangent vector is a scalar multiple of the position vector of the curve at that point.  Let's break it down:  1. **Tangent Vector**: The tangent vector to a curve at a point is a vector that "touches" the curve at that point and points in the direction in which the curve is going. For a unit-speed curve $\gamma(t)$, the tangent vector is given by $\gamma'(t)$.  2. **Position Vector**: The position vector of a point on the curve, relative to the origin, is simply $\gamma(t)$.  3. **Scalar Multiple**: Saying that the tangent vector is a scalar multiple of the position vector means there exists some scalar function $\lambda(t)$ such that $\gamma'(t) = \lambda(t) \gamma(t)$.  This relationship indicates that at every point on the curve, the direction in which the curve is moving (the tangent vector) is directly along the line from the origin to that point on the curve (the position vector), scaled by some factor $\lambda(t)$.  In simpler terms, if you draw a line from the origin to any point on the curve, the curve at that point is moving directly along this line, either towards or away from the origin, depending on the sign of $\lambda(t)$.   This behavior is characteristic of a straight line emanating from the origin. Hence, the curve must be part of a straight line.
% }}
The answer given by GPT-4 misses the point since it does not explain how the specific line the poster asks about follows from the assumptions.

% \begin{figure}
%     \centering
%     \begin{tcolorbox}[standard jigsaw,opacityback=0]
%     Imagine a car driving along the curve, and at the point of interest, the car hits an oil slick and shoots off in the straight line of its travel as it hits the point. The line of the car gives the tangent line at the point (provided the curve is differentiable at the point). You can look at cars sliding off coming from both directions to see the tangent line.
%     \end{tcolorbox}
%     \caption{Reason why GPT-4 guides retrieval in wrong direction}
%     \label{fig:extractedTOIs}
% \end{figure}

we observe a pattern that seems to be representative of how GPT-4-generated answers can guide the retrieval system in the wrong direction:\\ 
% \fbox{%
%   \parbox{0.47\textwidth}{
% Imagine a car driving along the curve, and at the point of interest, the car hits an oil slick and shoots off in the straight line of its travel as it hits the point. The line of the car gives the tangent line at the point (provided the curve is differentiable at the point). You can look at cars sliding off coming from both directions to see the tangent line.
%     }
% }
The retrieved answer only gives a general explanation of the concept of a tangent line to a curve. This corresponds to a portion of GPT-4's answer, which, tending to be verbose, also explains what a tangent line means.

\subsection{Tora-7b-Code \& Mistral-7b}
The answers obtained by all the smaller models (basically every model except GPT-4) are of quite low quality. 
The mathematical models exhibit the typical behavior of smaller models in that the prompt format is misunderstood and the answers lack coherence. Additionally, all models generate no output other than an end-of-sequence token for multiple questions. (6 in case of Tora-7b-Code).
In contrast, Mistral is much better in keeping a conversational tone than Tora. Additionally, the reasoning appears to be more structured. However, formulas are not written in latex format and are of lower quality, as apparent in the faulty input variables.
For both systems, there are individual cases where retrieval is significantly boosted.

\subsubsection{\href{https://math.stackexchange.com/questions/4212480/number-of-solutions-of-equation-over-a-finite-field?noredirect=1&lq=1}{A.309} - Tora-7b-Code boosts retrieval}
\begin{figure}
    \centering
    \begin{tcolorbox}[standard jigsaw,opacityback=0]
		I have a question regarding the number of solutions of a equation over a finite field $\mathbb{F}_p$. First of all, consider the equation $x^3=a$ over $\mathbb{F}_p$, where $p$ is a prime such that $p\equiv 2 (\text{mod }3)$. The book that I'm currently reading says that this equation has exactly one solution in $\mathbb{F}_p$ for every $a\in \mathbb{F}_p$, because $\gcd(3,p-1)=1$, but the book does not prove this. Unfortunately, this doesn't convince me enough. Is there is a convincing elementary straightforward proof justifying why is this true?
    \end{tcolorbox}
    \caption{ToRA improves precision}
    \label{fig:extractedTOIs}
\end{figure}

Compared to the following question, using the answer by Tora-7b-Code improves Precision@10 from 0.5 to 0.8.\\
% \fbox{%
%   \parbox{0.47\textwidth}{
% 		I have a question regarding the number of solutions of a equation over a finite field $\mathbb{F}_p$. First of all, consider the equation $x^3=a$ over $\mathbb{F}_p$, where $p$ is a prime such that $p\equiv 2 (\text{mod }3)$. The book that I'm currently reading says that this equation has exactly one solution in $\mathbb{F}_p$ for every $a\in \mathbb{F}_p$, because $\gcd(3,p-1)=1$, but the book does not prove this. Unfortunately, this doesn't convince me enough. Is there is a convincing elementary straightforward proof justifying why is this true?
%   }
% }
Here is the answer generated by Tora-7b-Code:

\begin{figure}
    \centering
    \begin{tcolorbox}[standard jigsaw,opacityback=0]
  Proof: Suppose to the contrary that there are more than one solution in $\mathbb{F}_p$. By Fermat's little theorem, $a^{p-1}=1$, then $a$ is congruent to $1$ modulo $p-1$. Since gcd$(3,p-1)=1$, there is a 
$k\in\mathbb{F}_p$ such that $3k\equiv 1$ mod $p-1$, then $a=(3k)^2\equiv 1$ mod $p-1$, which contradicts $a$ being in $\mathbb{F}_p$. Thus, the equation $x^3=a$ has exactly one solution in $\mathbb{F}_p$. $\blacksquare$ I don't really get the last part: "Since gcd$(3,p-1)=1$, there is a $k\in\mathbb{F}_p$ such that $3k\equiv 1$ mod $p-1$". Could you please elaborate on this part? Comment: I suggest you look into [this] ([...])  and [this]([...]). 
The way to show that an equation has exactly one solution in a finite field is usually by using the Chinese remainder theorem and the fact that if $a$ is a cube modulo $p$, then $a^{p-1}$ is congruent to $1$ modulo $p-1$. Comment: This actually is a question that came up in my intro to computation class and we couldn't find a simple proof for it. I am looking for a basic level proof.
Comment: If $p \equiv 2 \pmod{3}$, then $\gcd(p-1, 3) = 1$. By the Euclidean Algorithm, there is some $k \in \mathbb{F}_p$ such that $3k \equiv 1 \pmod{p-1}$. Therefore, $a \equiv k^2 \pmod{p-1}$. This contradicts [...]
    \end{tcolorbox}
    \caption{ToRA Answer}
    \label{fig:extractedTOIs}
\end{figure}


% \fbox{%
%   \parbox{0.47\textwidth}{

%   Proof: Suppose to the contrary that there are more than one solution in $\mathbb{F}_p$. By Fermat's little theorem, $a^{p-1}=1$, then $a$ is congruent to $1$ modulo $p-1$. Since gcd$(3,p-1)=1$, there is a 
% $k\in\mathbb{F}_p$ such that $3k\equiv 1$ mod $p-1$, then $a=(3k)^2\equiv 1$ mod $p-1$, which contradicts $a$ being in $\mathbb{F}_p$. Thus, the equation $x^3=a$ has exactly one solution in $\mathbb{F}_p$. $\blacksquare$ I don't really get the last part: "Since gcd$(3,p-1)=1$, there is a $k\in\mathbb{F}_p$ such that $3k\equiv 1$ mod $p-1$". Could you please elaborate on this part? Comment: I suggest you look into [this] ([...])  and [this]([...]). 
% The way to show that an equation has exactly one solution in a finite field is usually by using the Chinese remainder theorem and the fact that if $a$ is a cube modulo $p$, then $a^{p-1}$ is congruent to $1$ modulo $p-1$. Comment: This actually is a question that came up in my intro to computation class and we couldn't find a simple proof for it. I am looking for a basic level proof.
% Comment: If $p \equiv 2 \pmod{3}$, then $\gcd(p-1, 3) = 1$. By the Euclidean Algorithm, there is some $k \in \mathbb{F}_p$ such that $3k \equiv 1 \pmod{p-1}$. Therefore, $a \equiv k^2 \pmod{p-1}$. This contradicts [...]

%     }
% }
In lieu of an actual answer, it seems that Tora simulates a thread. As an answer, it is quite incoherent in addition to being logically false.
% The first retrieved answer for the original is the following: \\
% \fbox{%
%   \parbox{0.47\textwidth}{

% "Generically", the number of solutions (mod $p^a$) will be the same as the number of solutions (mod $p$). (There are exceptions though.)\\
% Without knowing it, you are looking for the magic of \href{https://en.wikipedia.org/wiki/Hensel\%27s_lemma}{Hensel's Lemma}!
% }
% }
% It misses the topic. However, prompted with the answer from Tora-7b-Code, the following relevant answer is retrieved: \\
% \fbox{%
%   \parbox{0.47\textwidth}{

% For $p \equiv 1 ($mod $3)$. Use the fact that $-3$ is a quadratic residue for $p$ to show that there are exactly three solutions for $x^3-1 \equiv 0 ($mod $p)$. The key step is to make use of the identity $4(x^2+x+1)=(2x+1)^2+3$. Then we can conclude there are exactly $(p-1)/3$ non-zero cubic residues. All of them have to satisfy the equation $x^{(p-1)/3}-1 \equiv 0 ($mod $p)$. Since there are at most $(p-1)/3$ solutions for $x^{(p-1)/3}-1 \equiv 0 ($mod $p)$, the set of non-zero cubic residues coincides with the set of the solutions. 

% For $p \equiv 2 ($mod $3)$, Bezout's lemma gives us $a,b \in \mathbb{Z}$ such that $1=3a+(p-1)b$. For any $r$, $r \equiv r^{(3a+(p-1)b)} \equiv r^{3a} \equiv (r^a)^3 $mod $p$.

% }}.
% We hypothesize that, even though the answer given by Tora is wrong and incoherent, it mentions the core question sufficiently often to boost retrieval.

% \subsubsection{\href{https://math.stackexchange.com/questions/4088631/fourier-transform-of-function-1-vert-x-vert?noredirect=1&lq=1}{A.360} - Mistral-7b-Instruct boosts retrieval}
% Mistral performs better than Tora and the DPR (0.6 vs. 0.2 vs. 0.3) for the following question.\\
% \fbox{%
% \parbox{0.47\textwidth}{
% 		I am helping someone with highschool maths but I got stacked in a elementary geometry problem.I am given the equation of two straigh lines in the space $r\equiv \begin{cases} x=1 \\ y=1 \\z=\lambda -2 \end{cases}$ and $s\equiv\begin{cases} x=\mu \\ y=\mu -1 \\ z=-1\end{cases}$ and asked for some calculations. First I am asked the relative position of them so I get they are skew lines. After that I am asked for the distance between the two lines. In order to get the distance I have to calculate the line that is perpendicular to both of them in the "skewing" point, check the points where it touches the other two lines (sorry, not sure about the word in English) and calculate the module of this vector.Im having trouble calculating the perpendicular line. I know I can get the director vector using vectorial product, but  I'm not sure how to find a point so that I can build the line.
% }}\\
% This is the answer generated by Mistral-7b:\\
% \fbox{%
%  \parbox{0.47\textwidth}{
%    To calculate the distance between two skew lines, one approach is to find a line segment that is perpendicular to both of them. This line segment can be found by taking the cross product of their director vectors. Let's first find the director vectors for the given lines. Let $r(x)$ be the parametric equation of the first line, and $s(x)$ be the parametric equation of the second line. $r(x)$: $x = 1, y = 1, z = \lambda - 2$ $s(x)$: $x = \lambda, y =\mu - 1, z = -1$ The parametric equations for the director vectors are: $dirr(x) = (\partial x/\partial t)r(x) \partial y/\partial t)r(x) 
%    \partial z/\partial t)r(x) = (0) (1) (1) dirs(x) = (\partial x/\partial t)s(x) \partial y/\partial t)s(x) \partial z/\partial t)s(x) = (0) (1) (-1)$The cross product of these director vectors gives us the normal vector of the line perpendicular to both lines: $np(x) = dirr(x) × dirs(x) = (-1, -1, 2) $ Now we need to find a point where this line touches both lines. Let's call this point $p$ and define it as: $p.r(u) = 0 p.s(u) = 0$ where $u$ is the parameter of $np$. To solve this system of equations, we need to use matrix algebra. Define the matrix of coefficients as: [...]
% }}
% In contrast, the answer given by Tora (omitted) contradicts the original post. The difference in retrieval quality appears to result from this contradiction, as the DPR then retrieves mostly negative results.
